Towards Foundation Model on Temporal Knowledge Graph Reasoning

Temporal Knowledge Graphs (TKGs) store temporal facts with quadruple formats (s, p, o, t). Existing Temporal Knowledge Graph Embedding (TKGE) models perform link prediction tasks in transductive or semi-inductive settings, which means the entities, relations, and temporal information in the test graph are fully or partially observed during training. Such reliance on seen elements during inference limits the models' ability to transfer to new domains and generalize to real-world scenarios. A central limitation is the difficulty in learning representations for entities, relations, and timestamps that are transferable and not tied to dataset-specific vocabularies. To overcome these limitations, we introduce the first fully-inductive approach to temporal knowledge graph link prediction. Our model employs sinusoidal positional encodings to capture fine-grained temporal patterns and generates adaptive entity and relation representations using message passing conditioned on both local and global temporal contexts. Our model design is agnostic to temporal granularity and time span, effectively addressing temporal discrepancies across TKGs and facilitating time-aware structural information transfer. As a pretrained, scalable, and transferable model, POSTRA demonstrates strong zero-shot performance on unseen temporal knowledge graphs, effectively generalizing to novel entities, relations, and timestamps. Extensive theoretical analysis and empirical results show that a single pretrained model can improve zero-shot performance on various inductive temporal reasoning scenarios, marking a significant step toward a foundation model for temporal KGs.

==> latex/proof.tex <==
\begin{theorem}[Multi-Frequency Affine Scorer
%:compatibility $\Longleftrightarrow$ existence
]
\label{thm:multi-frequency}
Let assume
\begin{itemize}
    \item $T>1$ be an integer time horizon ;
    \item $d_{\mathrm{PE}}\ge T$ be an even positional–encoding dimension;
    \item $P_1,\dots ,P_m,$ such that $P_i\mid T$ for every $i=1,\dots ,m,$ be a family of positive integers.

    
\end{itemize}

For any integer $\tau$ define the (standard) sinusoidal positional encoding
\[
  [\mathrm{TE}(\tau)]_{2n}   = \sin(\omega_n\tau),
  \qquad
  [\mathrm{TE}(\tau)]_{2n+1} = \cos(\omega_n\tau),
  \qquad
  0\le n < \tfrac{d_{\mathrm{PE}}}{2},
\]
with arbitrary real frequencies $\omega_0,\dots ,\omega_{d_{\mathrm{PE}}/2-1}$.

\medskip
\noindent
\textbf{Data to be fitted.}  
Let
\[
  G = \{V_1,\dots,V_m\}\subset\mathbb{R}^{d_V}
\]
be $m$ fixed context vectors and, for each $i=1,\dots ,m$, let
\[
  g_i : \{0,1,\dots ,T-1\}\longrightarrow \mathbb{R}
\]
be a \emph{non-constant} sequence which we extend to all $\mathbb{Z}$ by $P_i$-periodicity:
\[
  g_i(\tau) := g_i\!\bigl(\tau\bmod P_i\bigr),
  \qquad \tau\in\mathbb{Z}.
\]

\medskip
\noindent
\textbf{Encoding matrices.}
\[
  M \;=\;
  \begin{pmatrix}
    \mathrm{TE}(0)^\top\\
    \mathrm{TE}(1)^\top\\
    \vdots\\
    \mathrm{TE}(T-1)^\top
  \end{pmatrix}
  \in\mathbb{R}^{T\times d_{\mathrm{PE}}},
  \qquad
  B^{(i)}
  =
  \begin{pmatrix}
    \mathrm{TE}(P_i)^\top    - \mathrm{TE}(0)^\top\\
    \mathrm{TE}(P_i+1)^\top  - \mathrm{TE}(1)^\top\\
    \vdots\\
    \mathrm{TE}(T-1+P_i)^\top- \mathrm{TE}(T-1)^\top
  \end{pmatrix}
  \in\mathbb{R}^{T\times d_{\mathrm{PE}}}.
\]
Stack them block-diagonally:
\[
  \widetilde B := \operatorname{diag}\!\bigl(B^{(1)},\dots ,B^{(m)}\bigr)
  \in\mathbb{R}^{mT\times m\,d_{\mathrm{PE}}}.
\]

\medskip
\noindent
\textbf{Full–row–rank remark.}  
The proofs below do \emph{not} require\footnote{We keep the comment because full rank can be useful for subsequent uniqueness or least-squares considerations.} the condition $\operatorname{rank}M=T$; nevertheless one may keep it to rule out degenerate data sets in which no non-constant target can ever be matched.

\bigskip
\noindent
Define
\[
  g:=
  \begin{pmatrix}
    g_1\\
    \vdots\\
    g_m
  \end{pmatrix}
  \in\mathbb{R}^{mT},
  \qquad
  w_{\mathrm{PE}}:=
  \begin{pmatrix}
    w_{\mathrm{PE}}^{(1)}\\
    \vdots\\
    w_{\mathrm{PE}}^{(m)}
  \end{pmatrix}
  \in\mathbb{R}^{m\,d_{\mathrm{PE}}}.
\]

\begin{enumerate}[label=\textup{(\Alph*)},leftmargin=*,itemsep=4pt]
  \item \textbf{Compatibility \((\mathcal{C})\).}\;  
        There exists $w_{\mathrm{PE}}\in\mathbb{R}^{m\,d_{\mathrm{PE}}}$ solving the linear system
        \[
          \boxed{\;
          \begin{pmatrix}
            I_m\!\otimes\! M \\[4pt]
            \widetilde B
          \end{pmatrix}
          w_{\mathrm{PE}}
          =
          \begin{pmatrix}
            g\\[3pt]0
          \end{pmatrix}}
          \tag{$\mathcal{C}$}
        \]
        where $I_m\otimes M$ is the block-diagonal Kronecker product whose $i$-th diagonal block equals $M$.
  \item \textbf{Existence of a scorer \((\mathcal{S})\).}\;  
        There exist parameters
        \[
          \theta
          \;=\;
          \bigl(W_{\mathrm{PE}},\,w_V,\,b\bigr)
          \in
          \mathbb{R}^{d_{\mathrm{PE}}\times m}
          \times\mathbb{R}^{d_V}
          \times\mathbb{R}
        \]
        such that the affine map
        \[
          f_\theta\bigl(V,\mathrm{TE}(\tau)\bigr)
          :=
          w_V^\top V
          \;+\;
          W_{\mathrm{PE}}^\top\,\mathrm{TE}(\tau)
          \;+\;
          b
          \;\in\mathbb{R}^{m}
        \]
        obeys, for each $i=1,\dots ,m$,
        \begin{enumerate}[label=\textup{(\roman*)}]
          \item $P_i$-periodicity in $\tau\in\mathbb{Z}$;
          \item non-constancy as a function of $\tau$;
          \item interpolation on the basic window:
                \[
                  \bigl[f_\theta\!\bigl(V_i,\mathrm{TE}(\tau)\bigr)\bigr]_i
                  \;=\;
                  w_V^\top V_i + g_i(\tau),
                  \qquad
                  0\le\tau<T.
                \]
        \end{enumerate}
\end{enumerate}

\begin{center}
\framebox{\(\mathcal{C}\;\Longleftrightarrow\;\mathcal{S}\)}
\end{center}

\bigskip
\noindent
When these equivalent conditions hold one may choose \emph{any} solution $w_{\mathrm{PE}}$ of~\((\mathcal{C})\), set
\[
  W_{\mathrm{PE}}
  :=
  \bigl[w_{\mathrm{PE}}^{(1)}\;\cdots\;w_{\mathrm{PE}}^{(m)}\bigr],
  \qquad
  b=0,
\]
and pick an arbitrary $w_V$; the resulting $\theta$ satisfies \(\mathcal{S}\).
\end{theorem}

\begin{proof}[Step-by-step proof of \(\mathcal{C}\Longleftrightarrow\mathcal{S}\)]
We write $w_{\mathrm{PE}}=(w_{\mathrm{PE}}^{(1)},\dots ,w_{\mathrm{PE}}^{(m)})$ with
each block $w_{\mathrm{PE}}^{(i)}\in\mathbb{R}^{d_{\mathrm{PE}}}$.

\smallskip
\hrule\smallskip
\noindent
\textbf{Part I: \(\mathcal{C}\;\Longrightarrow\;\mathcal{S}\).}

Assume a vector $w_{\mathrm{PE}}$ satisfies system~\((\mathcal{C})\).

\begin{enumerate}[label=\textbf{Step~\arabic*:},leftmargin=*,itemsep=6pt]
\item \emph{Values on the basic window.}\;
      The top block $(I_m\otimes M)w_{\mathrm{PE}}=g$ is equivalent to
      \[
        M\,w_{\mathrm{PE}}^{(i)} \;=\; g_i \Big|_{\,0\le\tau<T},
        \quad
        i=1,\dots ,m.
      \tag{1}
      \]
\item \emph{$P_i$-periodicity of each component.}\;  
      The block $\widetilde B\,w_{\mathrm{PE}}=0$ gives for every $i$
      \[
        B^{(i)}\,w_{\mathrm{PE}}^{(i)} = 0
        \;\Longrightarrow\;
        w_{\mathrm{PE}}^{(i)\top}
        \bigl(\mathrm{TE}(\tau+P_i)-\mathrm{TE}(\tau)\bigr)=0,
        \quad
        0\le\tau<T.
      \]
      Thus
      \[
        w_{\mathrm{PE}}^{(i)\top}\mathrm{TE}(\tau+P_i)
        =w_{\mathrm{PE}}^{(i)\top}\mathrm{TE}(\tau),
        \quad 0\le\tau<T.
        \tag{2}
      \]
      Replacing $\tau$ by $\tau+kP_i$ and iterating shows
      \[
        w_{\mathrm{PE}}^{(i)\top}\mathrm{TE}(\tau+kP_i)
        = w_{\mathrm{PE}}^{(i)\top}\mathrm{TE}(\tau),
        \quad
        \forall\tau\in\{0,\dots ,T-1\},\;k\in\mathbb{Z},
      \]
      i.e.\ $P_i$-periodicity on \emph{all} integers.
\item \emph{Identify the periodic function on $\mathbb{Z}$.}\;
      Combine~(1) with periodicity: for every $\tau\in\mathbb{Z}$
      \[
        w_{\mathrm{PE}}^{(i)\top}\mathrm{TE}(\tau)
        = g_i\!\bigl(\tau\bmod P_i\bigr).
        \tag{3}
      \]
\item \emph{Assemble the scorer.}\;
      Define
      \[
        W_{\mathrm{PE}}
        :=
        \bigl[w_{\mathrm{PE}}^{(1)}\;\cdots\;w_{\mathrm{PE}}^{(m)}\bigr],
        \qquad
        b:=0,
        \qquad
        \text{choose any }w_V\in\mathbb{R}^{d_V}.
      \]
      Then
      \[
        f_\theta\bigl(V,\mathrm{TE}(\tau)\bigr)
        =
        w_V^\top V
        +
        \begin{pmatrix}
          w_{\mathrm{PE}}^{(1)\top}\mathrm{TE}(\tau)\\[-1pt]
          \vdots\\[-1pt]
          w_{\mathrm{PE}}^{(m)\top}\mathrm{TE}(\tau)
        \end{pmatrix},
      \]
      whose $i$-th component equals the right-hand side of~(3).  
      Therefore:

      * it is $P_i$-periodic by construction;  
      * it is non-constant because each $g_i$ is non-constant;  
      * on $0\le\tau<T$, (3) reduces to \(w_{\!V}^{\top}V_i+g_i(\tau)\).

      Hence \(\mathcal{S}\) holds.
\end{enumerate}

\smallskip
\hrule\smallskip
\noindent
\textbf{Part II: \(\mathcal{S}\;\Longrightarrow\;\mathcal{C}\).}

Conversely, suppose parameters \(\theta=(W_{\mathrm{PE}},w_V,b)\) satisfy \(\mathcal{S}\).
Write the columns as
\(
  W_{\mathrm{PE}}=[\,w_{\mathrm{PE}}^{(1)}\mid\cdots\mid w_{\mathrm{PE}}^{(m)}].
\)

\begin{enumerate}[label=\textbf{Step~\arabic*:},leftmargin=*,itemsep=6pt]
\item \emph{Matching on the basic window.}\;
      Evaluating property~(iii) at $0\le\tau<T$ gives
      \[
        M\,w_{\mathrm{PE}}^{(i)} = g_i \Big|_{\,0\le\tau<T},
        \quad
        i=1,\dots ,m.
        \tag{4}
      \]
\item \emph{$P_i$-periodicity implies the $B^{(i)}$ equations.}\;
      Property (i) yields, for every integer $\tau$,
      \(
        w_{\mathrm{PE}}^{(i)\top}\mathrm{TE}(\tau+P_i)=
        w_{\mathrm{PE}}^{(i)\top}\mathrm{TE}(\tau)
      \).
      Specialising to $\tau=0,\dots ,T-1$ one obtains
      \(
        B^{(i)}\,w_{\mathrm{PE}}^{(i)}=0
      \).
\item \emph{Stack the blocks.}\;
      Collecting (4) for all $i$ and the $B^{(i)}$ equations in a single vector $w_{\mathrm{PE}}$ yields exactly system~\((\mathcal{C})\).  Thus \(\mathcal{C}\) holds.
\end{enumerate}

\smallskip
\hrule\smallskip
\noindent
Both directions are proven; therefore \(\mathcal{C}\Longleftrightarrow\mathcal{S}\).  
The final comment about choosing $(W_{\mathrm{PE}},w_V,b)$ is precisely the construction in Part I, Step 4.
\end{proof}




\begin{theorem}[Universal Compatibility under harmonically–aligned frequencies]%
\label{thm:compat-always}
Fix
\[
  T>1,\qquad d_{\mathrm{PE}}\ge T,\qquad
  P_1,\dots ,P_m\in\mathbb N,\;\;P_i\mid T.
\]

\medskip
\noindent
Let \(L:=\operatorname{lcm}(P_1,\dots ,P_m)\) and choose \emph{any} collection of
integers \(k_0,k_1,\dots ,k_{d_{\mathrm{PE}}/2-1}\).
Define the frequencies
\[
  \omega_n \;:=\; \frac{2\pi k_n}{L},
  \qquad 0\le n<\tfrac{d_{\mathrm{PE}}}{2},
\]
and build the usual sinusoidal positional encoding
\[
  [\mathrm{TE}(\tau)]_{2n}   = \sin(\omega_n\tau),
  \quad
  [\mathrm{TE}(\tau)]_{2n+1} = \cos(\omega_n\tau),
  \qquad \tau\in\mathbb Z.
\]

Form the matrices
\[
  M\;=\;
  \begin{pmatrix}\mathrm{TE}(0)^\top\\ \vdots\\ \mathrm{TE}(T-1)^\top\end{pmatrix}\in\mathbb R^{T\times d_{\mathrm{PE}}},
  \qquad
  B^{(i)}
  =
  \begin{pmatrix}
    \mathrm{TE}(P_i)^\top-\mathrm{TE}(0)^\top\\
    \vdots\\
    \mathrm{TE}(T-1+P_i)^\top-\mathrm{TE}(T-1)^\top
  \end{pmatrix}
  \in\mathbb R^{T\times d_{\mathrm{PE}}}.
\]

\textbf{Claim.}  For these frequencies every \(B^{(i)}\) vanishes identically; hence the stacked
compatibility system
\[
  \begin{pmatrix}
    I_m\otimes M \\[4pt] \mathrm{diag}(B^{(1)},\dots ,B^{(m)})
  \end{pmatrix}
  w_{\mathrm{PE}}
  =
  \begin{pmatrix}
    g\\[3pt]0
  \end{pmatrix}
  \tag{$\mathcal{C}$}
\]
is always solvable, regardless of the choice of \emph{any} target sequences
\(g_i\colon\{0,\dots ,T-1\}\to\mathbb R\).
\end{theorem}

\begin{proof}[Step-by-step proof]
\textbf{Step 1.  Encoding is \(L\)-periodic.}
Because \(\omega_n L=2\pi k_n\),
\[
  \sin(\omega_n(\tau+L))=\sin(\omega_n\tau),\quad
  \cos(\omega_n(\tau+L))=\cos(\omega_n\tau),
  \qquad\forall\tau\in\mathbb Z,
\]
so \(\mathrm{TE}(\tau+L)=\mathrm{TE}(\tau)\).

\smallskip
\textbf{Step 2.  Encoding is also \(P_i\)-periodic.}
Each \(P_i\) divides \(L\), hence \(\mathrm{TE}(\tau+P_i)=\mathrm{TE}(\tau)\).
Therefore
\[
  B^{(i)}=0\in\mathbb R^{T\times d_{\mathrm{PE}}},
  \qquad i=1,\dots ,m.
\]

\smallskip
\textbf{Step 3.  Compatibility collapses to a single block.}
With every \(B^{(i)}\) equal to zero, system \((\mathcal{C})\) becomes
\[
  (I_m\otimes M)\,w_{\mathrm{PE}} \;=\; g .
  \tag{$\mathcal{C}'$}
\]

\smallskip
\textbf{Step 4.  Solve the reduced system.}
Write \(w_{\mathrm{PE}}=(w_{\mathrm{PE}}^{(1)},\dots ,w_{\mathrm{PE}}^{(m)})\)
and \(g=(g_1,\dots ,g_m)\) with blocks in \(\mathbb R^{T}\).
The Kronecker structure of \(I_m\otimes M\) splits \((\mathcal{C}')\) into
\(m\) independent systems
\[
  M\,w_{\mathrm{PE}}^{(i)} = g_i,\qquad i=1,\dots ,m.
  \tag{$\mathcal{C}_i$}
\]
Because \(d_{\mathrm{PE}}\ge T\), the rows of \(M\) are linearly dependent
at worst; pick any right inverse \(M^{+}\) (for instance the Moore–Penrose
pseudoinverse).  Then
\[
  w_{\mathrm{PE}}^{(i)} := M^{+}g_i
  \quad (i=1,\dots ,m)
\]
solves each \((\mathcal{C}_i)\), and hence \(w_{\mathrm{PE}}\) solves the full
system \((\mathcal{C})\).

\smallskip
\textbf{Step 5.  Conclusion.}
Compatibility holds \emph{for every choice of data} \(\{g_i\}\)
once the frequencies obey \(\omega_n=\tfrac{2\pi k_n}{L}\).
\end{proof}
